Clifford algebra and the projective model of Minkowski (pseudo-Euclidean) spaces

I apply the algebraic framework introduced in arXiv:1101.4542v3[math.MG] to Minkowski (pseudo-Euclidean) spaces in 2, 3, and 4 dimensions. The exposition follows the template established in arXiv:1307.2917[math.MG] for Euclidean spaces. The emphasis is on geometric structures, but some contact with special relativity is made by considering relativistic addition of velocities and Lorentz transformations, both of which can be seen as rotation applied to points and to lines. The language used in the paper reflects the emphasis on geometry, rather than applications to special relativity. The use of Clifford algebra greatly simplifies the study of Minkowski spaces, since unintuitive synthetic techniques are replaced by algebraic calculations.

==> g-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-128.442176,23.532118)(-1.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-148.599027,124.642385)(-1.000000,-0.208337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-96.250702,205.382393)(-0.625000,0.000000){$\textbf{aI}$}


==> g-10.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-10_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-137.527515,209.781558)(-1.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-140.323521,88.265155)(0.000000,-0.500000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-55.134577,43.308183)(-1.000000,-0.023640){$(\textbf{P}\cdot\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-155.862415,143.016574)(-0.750000,0.226360){$(\textbf{P}\wedge\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-28.781789,173.440204)(0.000000,-0.500000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-23.367894,209.263834)(-0.750000,0.226360){$(\textbf{N}\cdot\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-67.987366,151.812415)(-0.250000,-0.773640){$(\textbf{N}\wedge\textbf{b})\textbf{b}^{-1}$}


==> g-11.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-11_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-39.793606,25.441306)(0.000000,0.000000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-165.919198,23.532118)(-1.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-193.296892,51.482941)(-1.000000,-0.250000){$\textbf{b}\textbf{a}\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-102.460996,213.049392)(-0.500000,0.218750){$\phi_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-63.353881,200.635287)(0.000000,0.218750){$\phi_2$}


==> g-12.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-12_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-165.919198,23.532118)(-1.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-147.463474,101.253520)(-1.000000,-0.750000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-50.409577,52.441525)(-0.500000,-1.000000){$\textbf{b}\textbf{N}\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-170.099124,84.924075)(0.000000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-56.532392,141.707441)(0.000000,-0.814617){$\textbf{b}\textbf{Q}\textbf{b}^{-1}$}


==> g-13.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-13_0.pdf}%
}%
\special{pdf:q}%
\begin{picture}( 233.062738, 233.313676)%
\special{pdf:\ASYraw{
 -232.192018 0.250000 m
 -0.250000 0.250000 l
 -0.250000 232.192018 l
 -232.192018 232.192018 l
 -232.192018 0.250000 l
h
W n
}%
}%
\special{pdf:\ASYraw{
 -232.192018 -450.752437 m
 -0.250000 -450.752437 l
 -0.250000 683.194455 l
 -232.192018 683.194455 l
 -232.192018 -450.752437 l
h
W n
}%
}%
\special{pdf:q}%
\special{pdf:\ASYraw{
 -232.192018 0.250000 m
 -0.250000 0.250000 l
 -0.250000 232.192018 l
 -232.192018 232.192018 l
 -232.192018 0.250000 l
h
W n
}%
}%
\special{pdf:\ASYraw{
 -232.192018 -96.861006 m
 -0.250000 -96.861006 l
 -0.250000 329.303024 l
 -232.192018 329.303024 l
 -232.192018 -96.861006 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.997917,119.997917)(-1.000000,0.000000){$\textbf{S}$}
\special{pdf:Q}%
\end{picture}%
\kern -233.062738pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-119.997917,176.781283)(-1.000000,0.220820){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.997917,63.214551)(-1.000000,0.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-176.781283,119.997917)(-1.000000,0.000000){$\textbf{U}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-56.532392,113.315758)(0.000000,-1.000000){$\textbf{R}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-38.415363,163.823250)(0.000000,-0.450000){$B\textbf{R}\!B^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-71.852926,194.898313)(-0.700000,0.185383){$B\textbf{Q}\!B^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-158.625750,43.140363)(0.000000,-0.500000){$B\textbf{P}\!B^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-185.448313,69.962926)(0.000000,-0.500000){$B\textbf{U}\!B^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-62.573472,11.891528)(-1.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-142.108933,11.782256)(-1.000000,-0.500000){$B\textbf{b}B^{-1}$}


==> g-14.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-14_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-105.581291,139.938018)(0.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-84.924075,56.532392)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-140.656312,69.173209)(-0.500000,-0.833337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-47.520300,163.219198)(0.000000,-0.500000){$T\textbf{b}T^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-27.701789,93.462655)(-0.136364,0.000000){$T\textbf{P}T^{-1}$}


==> g-15+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-15+0_0.pdf}%
}%


==> g-15.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-15+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -403.040035652651283726,3Droll=0,3Droo=403.040035652651283726,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-15+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-15+0.prc}}


==> g-16+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-16+0_0.pdf}%
}%


==> g-16.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 231.257250pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,115.628625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-16+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-16+0.js]{254.9525pt}{228.855pt}{\ASYprefix\jobname-16+0.prc}}


==> g-17+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-17+0_0.pdf}%
}%


==> g-17.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-17+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-17+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-17+0.prc}}


==> g-18+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-18+0_0.pdf}%
}%


==> g-18.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-18+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-18+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-18+0.prc}}


==> g-19+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-19+0_0.pdf}%
}%


==> g-19.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 238.283510pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,119.141755)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-19+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -416.74248361619845582,3Droll=0,3Droo=416.74248361619845582,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-19+0.js]{254.9525pt}{235.88125pt}{\ASYprefix\jobname-19+0.prc}}


==> g-2.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-83.260857,22.450605)(0.000000,-0.100000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-166.084655,77.114584)(-1.000000,-0.762071){$\textbf{e}_0\wedge\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-133.897950,180.280497)(-0.100000,0.000000){$\textbf{bI}$}


==> g-20+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-20+0_0.pdf}%
}%


==> g-20.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-20+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-20+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-20+0.prc}}


==> g-21+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-21+0_0.pdf}%
}%


==> g-21.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-21+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.93199915605617889,3Droll=0,3Droo=410.93199915605617889,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-21+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-21+0.prc}}


==> g-22+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-22+0_0.pdf}%
}%


==> g-22.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-22+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.93199915605617889,3Droll=0,3Droo=410.93199915605617889,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-22+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-22+0.prc}}


==> g-23+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-23+0_0.pdf}%
}%


==> g-23.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-23+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-23+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-23+0.prc}}


==> g-24+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-24+0_0.pdf}%
}%


==> g-24.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-24+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-24+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-24+0.prc}}


==> g-25+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-25+0_0.pdf}%
}%


==> g-25.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 232.261000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,116.130500)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-25+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.93199915605617889,3Droll=0,3Droo=410.93199915605617889,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-25+0.js]{254.9525pt}{229.85875pt}{\ASYprefix\jobname-25+0.prc}}


==> g-26+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-26+0_0.pdf}%
}%


==> g-26.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 232.261000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,116.130500)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-26+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-26+0.js]{254.9525pt}{229.85875pt}{\ASYprefix\jobname-26+0.prc}}


==> g-27+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-27+0_0.pdf}%
}%


==> g-27.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-27+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.93199915605617889,3Droll=0,3Droo=410.93199915605617889,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-27+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-27+0.prc}}


==> g-28+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-28+0_0.pdf}%
}%


==> g-28.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-28+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.93199915605600836,3Droll=0,3Droo=410.93199915605600836,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-28+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-28+0.prc}}


==> g-29+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-29+0_0.pdf}%
}%


==> g-29.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-29+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056576794,3Droll=0,3Droo=410.931999156056576794,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-29+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-29+0.prc}}


==> g-3.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-185.292901,107.711797)(-0.250000,-1.000000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-145.612934,174.569029)(-0.750000,0.166663){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-91.606234,119.997917)(-1.000000,0.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-44.117748,210.989035)(-1.000000,-0.250000){$\textbf{a}\cdot\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-61.159600,86.208219)(-0.500000,-0.750000){$\textbf{e}_0\wedge(\textbf{a}\cdot\textbf{P})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-69.509646,132.896421)(-0.250000,-0.750000){0.447214 0.894427 -0.894427 0.447214}{$|\textbf{a}\vee\textbf{P}|$}


==> g-30+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-30+0_0.pdf}%
}%


==> g-30.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-30+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.931999156056235734,3Droll=0,3Droo=410.931999156056235734,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-30+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-30+0.prc}}


==> g-4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-91.606234,119.997917)(-1.000000,0.000000){\textbf{P}}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-63.214551,176.781283)(-1.000000,0.220820){\textbf{Q}}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-44.402795,209.781558)(-1.000000,-0.279180){$\textbf{P}\vee\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-37.160125,74.208482)(-0.500000,-0.750000){$\textbf{e}_0\wedge(\textbf{P}\vee\textbf{Q})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-72.160125,33.390977)(0.000000,0.220820){$\textbf{P}\times\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-69.509646,132.896421)(-0.250000,-1.000000){0.447214 0.894427 -0.894427 0.447214}{$\norm{\textbf{P}\vee\textbf{Q}}$}


==> g-5.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-5_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-113.315758,56.532392)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-84.924075,170.099124)(0.000000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-70.728234,113.315758)(0.000000,-1.000000){$\textbf{R}$}


==> g-6.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-6_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-185.244228,192.431596)(-0.952574,0.097769){0.800000 0.000000 0.000000 0.800000}{\vphantom{$10^4$}$-1.5$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-178.582044,197.966818)(-0.880797,0.097769){0.800000 0.000000 0.000000 0.800000}{\vphantom{$10^4$}$-1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-159.531309,209.435196)(-0.731059,0.097769){0.800000 0.000000 0.000000 0.800000}{\vphantom{$10^4$}$-0.5$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-116.656838,218.862728)(-0.500000,0.000000){0.800000 0.000000 0.000000 0.800000}{\vphantom{$10^4$}$0$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-73.782367,209.435196)(-0.268941,0.000000){0.800000 0.000000 0.000000 0.800000}{\vphantom{$10^4$}$0.5$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-54.731632,197.966818)(-0.119203,0.000000){0.800000 0.000000 0.000000 0.800000}{\vphantom{$10^4$}$1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-48.069448,192.431596)(-0.047426,0.000000){0.800000 0.000000 0.000000 0.800000}{\vphantom{$10^4$}$1.5$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-90.910534,46.813298)(0.000000,-0.091464){$\begin{aligned}&\phi=-0.3\\ &d=0\end{aligned}$}


==> g-7.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-7_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-50.034334,126.832466)(-0.500000,-1.000000){$\textbf{N}=\textbf{a}\wedge\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-187.354193,146.840467)(-0.666667,-1.000000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-102.925879,157.849715)(-0.333333,0.166663){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-187.354193,71.129313)(-0.666667,-1.000000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-127.843040,89.848231)(-0.750000,0.137929){$\textbf{e}_0\wedge\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-66.371041,59.074496)(-1.000000,0.125000){0.316228 -0.948683 0.948683 0.316228}{$|\textbf{e}_{12}\vee\textbf{N}|$}


==> g-8.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-8_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-109.213974,149.104476)(-1.000000,-0.500000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-190.450415,25.029808)(-1.000000,-0.166667){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-63.697534,123.710182)(0.000000,-0.333337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-48.773984,31.637113)(-1.000000,-0.750000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-69.005082,165.496421)(0.000000,-0.362071){$\textbf{e}_0\wedge\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-101.401075,201.395529)(-0.500000,0.218750){$\phi_{ab}$}


==> g-9.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-9_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.093763)(-1.000000,-0.500000){$t$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-137.527515,209.781558)(-1.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-99.760996,209.781558)(0.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-44.117748,22.324641)(-1.000000,-0.523640){$(\textbf{a}\cdot\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-183.800378,188.418212)(0.000000,-0.023640){$(\textbf{a}\wedge\textbf{b})\textbf{b}^{-1}$}

